Witness-Functions versus Interpretation-Functions for Secrecy in Cryptographic Protocols: What to Choose?

Proving that a cryptographic protocol is correct for secrecy is a hard task. One of the strongest strategies to reach this goal is to show that it is increasing, which means that the security level of every single atomic message exchanged in the protocol, safely evaluated, never deceases. Recently, two families of functions have been proposed to measure the security level of atomic messages. The first one is the family of interpretation-functions. The second is the family of witness-functions. In this paper, we show that the witness-functions are more efficient than interpretation-functions. We give a detailed analysis of an ad-hoc protocol on which the witness-functions succeed in proving its correctness for secrecy while the interpretation-functions fail to do so.

==> rappelSomeConf.tex <==
\section{On the correctness of increasing protocols}\label{sectionPreuveThFond}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       

Hereafter, we remind an important result: ''A protocol keeps its secret inputs when analyzed with a safe function and shown increasing''.

\subsection{Safe functions}
\begin{defini}{(Well-formed Function)}\label{bienforme}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. ${F}$ is ${\mathcal{C}}$-well-formed iff:
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}) \mbox{:}$\\

\begin{tabular}{lll}
   ${F}(\alpha,\{\alpha\})$ & $=$ & $\bot$ \\
   ${F}(\alpha, {M}_1 \cup {M}_2)$ & $=$ & ${F}(\alpha, {M}_1)\sqcap{F}(\alpha,{M}_2)$ \\
   ${F}(\alpha,{M})$ & $=$ & $\top, \mbox{ if } \alpha \notin {\mathcal{A}}({M})$ \\
\end{tabular}
}$ $\\
\end{defini}

A well-formed function ${F}$ must return the infimum to an atom $\alpha$ that appears  clear in $M$ to say that  any participant knows it from $M$. It  returns to an atom in the union of two sets, the minimum of the two values calculated in each set separately. It returns the supremum to any atom $\alpha$ that does not appear in $M$ to say that nobody could get it from $M$.\\

\begin{defini}{(Full-Invariant-by-Opponent Function)}\label{spi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. 
${F}$ is full-invariant-by-Opponent iff: $\forall {M} \subseteq {\mathcal{M}}, m\in {\mathcal{M}},  \alpha \in {\mathcal{A}}(m)$:\\
$
 {M} \models_{\mathcal{C}} m \Rightarrow ({F}(\alpha,m) \sqsupseteq{F}(\alpha,{M})) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner).
$\\
}
\end{defini}

A full-invariant-by-opponent function ${F}$ is such, when it affects a security level to an atom $\alpha$ in a set of messages $M$, the opponent cannot deduce from this set some message $m$ in which this level decreases (i.e. ${F}(\alpha,m) \not \sqsupseteq{F}(\alpha,{M})$), unless he is expressly entitled  to know it (i.e. $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$).\\

A function ${F}$ is s said to be safe if it is well-formed and full-invariant-by-Opponent.\\



\begin{defini}{(${F}$-Increasing Protocol)}\label{ProAbsCroi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification and $p$ be a protocol.\\
$p$ is ${F}$-increasing iff: $\forall R.r \in R_G(p), \sigma \in \Gamma,  \alpha \in {\mathcal{A}}(r^+), \mbox{ we have: }{F}(\alpha, r^+\sigma)\sqsupseteq \ulcorner \alpha \urcorner \sqcap{F}(\alpha, R^-\sigma)$
}
\end{defini}
$ $\\
An ${F}$-increasing protocol must produce traces with atomic messages having always a security level, returned by ${F}$, higher when sending (i.e. in $ r^+\sigma$) than when receiving (i.e. in $R^-\sigma$) or than its level set in the context (i.e. $\ulcorner \alpha \urcorner$), if known. \\


\begin{thm}{(Sececy in Increasing Protocols)}\label{mainTh}
{
Let ${F}$ be a safe function and $p$ be an ${F}$-increasing protocol.
\begin{center}
$p$ keeps its secret inputs.
\end{center}
}
\end{thm}
$ $\\

Theorem \ref{mainTh} states that a protocol keeps its secret inputs when it is analyzed by a safe function $F$ and is shown increasing. This result is quite intuitive. In fact, if the opponent succeeds to obtain a secret $\alpha$ (clear) from the protocol then its security level given  by $F$ is the infimum since $F$ is well-formed. That cannot be due to the rules of the protocol  since this latter is $F\mbox{-increasing}$. That could not arise neither when the opponent uses his capabilities since $F$ is full-invariant-by-opponent. So, the secret is kept forever. The detailed proof is available in~\cite{Relaxed}.

\section{Guideline for Building Safe Functions}\label{sectionFonctionsetSelections}


In ~\cite{WitnessArt1} we propose a class  of safe selections: $S_{Gen}^{EK}$. Any selection $S$ in $S_{Gen}^{EK}$ must return to an atom $\alpha$ in a message $m$:

\begin{enumerate}
\item if $\alpha$ is encrypted by a key $k$ such that $k$ is the outer key that satisfies the condition $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ (we refer to it by the external protective key), a subset among $k^{-1}$ and the neighbors of $\alpha$ under the same protection by $k$;
\item for two messages linked by a function $f$ in $\Sigma$ other than an encryption by a protective key (e.g. pair), the union of two subselections in these two messages.
\item if $\alpha$ does not have a protective key in $m$, the infimum (all atoms);
\item if $\alpha$ does not appear in $m$, the supremum (the empty set);
\end{enumerate}

%%We prove that any $S\in S_{Gen}^{EK}$ is ${\mathcal{C}}$-safe.\\

Among the selections of $S_{Gen}^{EK}$, we spotlight three practical ones:
\begin{enumerate}
\item the selection $S_{MAX}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$, all the principal identities inside the same protection by $k$, in addition to $k^{-1}$;
\item the selection $S_{EK}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$,  the key $k^{-1}$;
\item the selection $S_{N}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the key external protective key $k$, all the principal identities inside the same protection by $k$;
\end{enumerate}
Any selection $S$ in $S_{Gen}^{EK}$ when composed to a adequate homomorphism $\psi$ returns a safe function $F=\psi \circ S$. 
We choose the homomorphism that returns for:
\begin{enumerate}
\item an agent, its identity;
\item the key $k^{-1}$, if selected, the set of agent identities  that are authorized to know it.
\end{enumerate}
We denote by $F_{MAX}^{EK}, F_{EK}^{EK}$ and $F_{N}^{EK}$ respectively the functions resulting from the compositions $\psi \circ S_{MAX}^{EK}, \psi \circ S_{EK}^{EK}$ and $\psi \circ S_{N}^{EK}$. We prove~\cite{WitnessArt1} that these functions are safe. In fact, since the selection for any atom $\alpha$  is performed in an invariant section protected by the external protective key $k$, then, to alter this section (to decrease the security level of  $\alpha$), the opponent must have priorly obtained the atomic key $k^{-1}$. At this point of the proof, his knowledge must satisfy: $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner$. Since the key $ k^{-1}$ satisfies: $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ then the knowledge of the opponent must satisfy $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ too seeing that the comparator "$\sqsupseteq$" is transitive. This is simply the definition of a full-invariant-by-opponent function. These functions are well-formed by construction, too. 
%%\end{comment}


\begin{exemple}$ $\\

Context: $\ulcorner \alpha \urcorner=\{A, B, S\}$; $m=\{C.\{\alpha.D\}_{k_{as}}\}_{k_{ab}}$; ${k_{ab}^{-1}}={k_{ab}}, {k_{as}^{-1}}={k_{as}}$; $\ulcorner{k_{as}}\urcorner=\{A, S\}, \ulcorner{k_{ab}}\urcorner=\{A, B\}$. We have: \\
$S_{MAX}^{EK}(\alpha,m)=\{C, D, {k_{ab}^{-1}}\}$ and $F_{MAX}^{EK}(\alpha,m)=\psi\circ S_{MAX}^{EK}(\alpha,m)=\{C, D\}{ \cup}\ulcorner{k_{ab}^{-1}}\urcorner=\{C,D\} \cup \{A,B\}=\{A, B, C, D\}$.
\end{exemple} $ $\\

%%In all that follows, we refer to  any of the functions above by $F$ .

\section{Witness functions to eliminate the effect of variables}\label{sectionWF}

The functions  $F\in\{F_{MAX}^{EK}, F_{EK}^{EK}, F_{N}^{EK}\}$ we have  defined so far are not useful in practice since they operate on ground terms only. However, a static analysis should be run over messages of the generalized roles resulting from writing the protocol in a role-based specification~\cite{Debbabi11}. These messages contain variables that denote a content that an agent ignores and on which he cannot perform any verification. We give here a safe way to deal with variables. But now, let us  introduce derivation in Definition \ref{derivation}.$ $\\ %% as shown in \ref{derivation}. 
%%\pagebreak

\begin{defini}{[Derivation]}\label{derivation}
%%A derivative message is defined by the following rules:
%%\begin{table}[h]
%% \centering
\begin{center}
\begin{tabular}{rrcll}
~~~~~~& $\partial_X \alpha$ & $=$ & $\alpha$ &\\
& $\partial_X X$ & $=$& $\epsilon$ &\\
& $\!\!\partial_X Y~$ & $=$ & $Y, X\not = Y$ &\\
& $\partial{[\overline{X}]} m$ & $=$ & $\partial_{\{{\mathcal{X}}_m\backslash \{X\}\}} m$ &\\
& $\partial_X f(m)$ & $=$ & $ {f}(\partial_X m), f\in \Sigma$ &\\
& $\partial_{S_1 \cup S_2}m$ & $=$& $\partial_{S_1}\partial_{S_2}m$&\\ \\
\end{tabular}
\end{center}
%%\end{table}
\end{defini}

Derivation simply eliminates variables from a message except a variable under evaluation. The expression $\partial m$ denotes a message $m$ after removing all variables in. The aim of derivation is to deprive  variables from playing any role when evaluating an atom in a message. The idea  is hence to apply $F$ on the derivative message instead of the message itself. Besides, any variable is evaluated as a block with no regard to its content (i.e quantified). In fact, the reason why we do not care about the content of a variable is that if a variable, globally evaluated, is shown increasing that means that it cannot be discovered by any unauthorized party, and consequently any content inside cannot be discovered by an unauthorized party, too. If it is not increasing, then the protocol will not satisfy our sufficient conditions and hence no decision with respect to secrecy is made on, thus, with respect to authentication, too. This way of treating variables allows us to  give any content of a variable (dynamically known) the same value of the variable itself (statically calculable). The way we evaluate an atom from within a derivative message is described by Definition \ref{Fder}. $ $ \\
\begin{defini}\label{Fder}
$ $\\
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.\\
For all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, we denote by:
\[
F(\alpha, \partial [\overline{\alpha}] m\sigma) = \left\{
\begin{array}{ll}
F(\alpha,\partial m) & \mbox{if } \alpha \in {\mathcal{A}}(\partial m),\\
F(X,\partial [\overline{X}] m) & \mbox{if }\alpha \notin {\mathcal{A}}(\partial m) \\
%% & \mbox{and } \alpha \in {\mathcal{A}}(X\sigma). \\
& \mbox{and } \alpha =X\sigma. 
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma).\\
%% \underset{X \in {{\mathcal{X}}_m} } {\sqcap}

%% \mbox{ if } \alpha \not \in {\mathcal{A}}(\partial m) \mbox{ and }\alpha \in {\mathcal{A}}(X\sigma). \\
%% \\
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma). \\

\end{array}
\right.
\]
\end{defini}

Since the expression $F(\alpha, \partial [\overline{\alpha}] m\sigma)$ does not depend on substitution (i.e the run $\sigma$), we denote it simply by $F'(\alpha,m)$. Although the derivative function $F'$ allows us to neutralize variables, which is as such an important intermediate result, using it as is to analyze protocols is not safe because it is not even a function in the protocol. In fact, when we want to evaluate the security level of $\alpha$ in the trace $\{\alpha.A.B\}_{k_{cd}}­$ for example, we must return to the generalized roles to see from which message (with variables) this trace is generated and we may realize that more than one message are able to generate it. For instance, the messages $m_1=\{\alpha.A.X\}_{k_{cd}}­$ and $m_2=\{\alpha.Y.B\}_{k_{cd}}­$ are both candidates to generate the trace $\{\alpha.A.B\}_{k_{cd}}­$ (i.e. possible sources of it). If we refer to the first source (i.e. to $m_1$), the security level of $\alpha$ returned by $F'$ (with $F=F_{MAX}^{EK}$) is: 
$$F'(\alpha,\{\alpha.A.X\}_{k_{cd}})=F(\alpha,\{\alpha.\textcolor{red}{A}\}_{k_{\textcolor{red}{cd}}})=\{A, C, D\}$$
Whereas, if we refer to the second source (i.e. to $m_2$), its security level  is: 
$$F'(\alpha,\{\alpha.Y.B\}_{k_{cd}})=F(\alpha,\{\alpha.\textcolor{magenta}{B}\}_{k_{\textcolor{magenta}{cd}}})=\{B, C, D\}$$
Therefore, we cannot rely on $F'$ to analyze a protocol. To overcome this insufficiency, we define the witness functions. A witness function  looks for  all the sources of a ground term $m\sigma$ in the finite set  ${\mathcal{M}}_p^{\mathcal{G}}$, applies $F'$ to all of them, and returns the minimum. This minimum must satisfy both existence and uniqueness in the security lattice. Since a secret is always evaluated under the protection of a protective key, the research  of the  sources of a closed message in ${\mathcal{M}}_p^{\mathcal{G}}$ is then restricted to encryption patterns. We denote by  $\tilde{\mathcal{M}}_p^{\mathcal{G}}$ the set of all  encryption patterns generated by the protocol (renamed).\\


\begin{comment}
Let us see the problem in Example \ref{exempleApp}.

\begin{exemple}\label{exempleApp}
Let $m_1$ and $m_2$ be two messages of a generalized role such that 
$m_1=\{\alpha.C.X\}_{k_{ab}}$ and $m_2=\{\alpha.Y.S\}_{k_{ab}}$ and $\ulcorner\alpha\urcorner=\{A,B,S\}$ and $\ulcorner{k_{ab}^{-1}}\urcorner=\{A,B\}$. Let $m=\{\alpha.C.S\}_{k_{ab}}$ be a valid trace. Let $F=F_{MAX}^{EK}$.\\
$$F'(\alpha, m)=\begin{cases}
F'(\alpha, m_1\sigma_1)=\{A, B, C\}&| X\sigma_1=S\\
F'(\alpha, m_2\sigma_2)=\{A, B, S\}&| Y\sigma_2=C
\end{cases}$$
\end{exemple}

Thus, $F'$ is not compulsorily a function since it might return more than one output for the same input. 
\end{comment}




\begin{defini}{[witness function]}\label{WF}
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.
Let $p$ be a protocol and $F$ be a safe function. 
We define a witness function ${\mathcal{W}}_{p,F}$ for all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, as follows: 
%%On définit la fonction témoin sur les messages clos comme suit: 
\[{{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)=\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha, m'\sigma')\]
%%${\mathcal{W}}_{p,F}$ is said to be a witness function inside a protective key when $F$ is a verification Function such that its associated selection is an instance of the class $\Upsilon_{Gen}.$\\
\end{defini}

%%As we could see, a witness function depends on the set of sources of $m\sigma$ in ${\mathcal{M}}_p^{\mathcal{G}}$ (i.e. the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma|m'\sigma' = m \sigma\}$). So it depends on the substitution $\sigma$ that is not statically known. For that, we bind the witness function into two bounds that are independent of all substitution (runs). These bounds are provided by Lemma \ref{prePAT}.

Using a witness function as is to analyze a protocol is a very tedious  process since we cannot enumerate all the valid traces $m\sigma$ and their sources statically. For that we bind it into two bounds that do not depend on substitution (i.e on $\sigma$). The upper bound of a witness function returns a minimum set of confirmed principal identities for any $\alpha$ in $m$ whereas the lower bound returns the set of all principal identities from all the possible sources of $m$ (that are unifiable with it) including the odd ones.  The lower bound hunts so any odd principal identity and interprets it as an attack. The proof is simple since we have always  $\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma \} \subseteq \{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma' \}$ in the security lattice whatever $\sigma$. This is expressed by Proposition~\ref{prePAT}.\\

\begin{pre}{[binding a witness function]}\label{prePAT}
Let $m\in{\mathcal{M}}_p^{\mathcal{G}}$. Let ${\mathcal{W}}_{p,F}$ be a witness function.
For all $\sigma \in \Gamma$ we have:
$$F'(\alpha, m)\sqsupseteq {{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)\sqsupseteq \!\!\!\! \!\!\!\! \!\!\! \underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha, m'\sigma')$$
\end{pre}



\section{Sufficient conditions for authentication (Contribution)} \label{suffCondAuth}

The Lemma \ref{PAT} declares a decision criterion for secrecy  based on the bounds  of a witness function. The upper bound returns the set of original and trusted identities only from the received message. The lower bound returns the set of all the identities including those that could be inserted by a masquerader by substituting a regular message when sent. The criterion makes sure that no odd identity could be inserted in the evaluation neighborhood of a given  atom in the sent message.  The  proof  of Lemma \ref{PAT} results directly from Proposition \ref{prePAT} and Theorem \ref{mainTh}. \\

\begin{thm}{[Decision for Secrecy]}\label{PAT}
Let $p$ be a protocol. Let ${\mathcal{W}}_{p,F}$ be a witness function.
$p$ is correct with respect to secrecy if:
$\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$ we have:
$$\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = r^+ \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha,  m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F'(\alpha, R^-)$$
\end{thm}



==> rappelTrustCom.tex <==
\section{On the correctness of increasing protocols}\label{sectionPreuveThFond}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       

Hereafter, we remind an important result: ''A protocol keeps its secret inputs when analyzed with a safe function and shown increasing''.

\subsection{Safe functions}
\begin{defini}{(Well-formed Function)}\label{bienforme}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. ${F}$ is ${\mathcal{C}}$-well-formed iff:
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}) \mbox{:}$\\

\begin{tabular}{lll}
   ${F}(\alpha,\{\alpha\})$ & $=$ & $\bot$ \\
   ${F}(\alpha, {M}_1 \cup {M}_2)$ & $=$ & ${F}(\alpha, {M}_1)\sqcap{F}(\alpha,{M}_2)$ \\
   ${F}(\alpha,{M})$ & $=$ & $\top, \mbox{ if } \alpha \notin {\mathcal{A}}({M})$ \\
\end{tabular}
}$ $\\
\end{defini}

A well-formed function ${F}$ must return the infimum to an atom $\alpha$ that appears  clear in $M$ to say that  any participant knows it from $M$. It  returns to an atom in the union of two sets, the minimum of the two values calculated in each set separately. It returns the supremum to any atom $\alpha$ that does not appear in $M$ to say that nobody could get it from $M$.\\

\begin{defini}{(Full-Invariant-by-Opponent Function)}\label{spi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. 
${F}$ is full-invariant-by-Opponent iff: $\forall {M} \subseteq {\mathcal{M}}, m\in {\mathcal{M}},  \alpha \in {\mathcal{A}}(m)$:\\
$
 {M} \models_{\mathcal{C}} m \Rightarrow ({F}(\alpha,m) \sqsupseteq{F}(\alpha,{M})) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner).
$\\
}
\end{defini}

A full-invariant-by-opponent function ${F}$ is such, when it affects a security level to an atom $\alpha$ in a set of messages $M$, the opponent cannot deduce from this set some message $m$ in which this level decreases (i.e. ${F}(\alpha,m) \not \sqsupseteq{F}(\alpha,{M})$), unless he is expressly entitled  to know it (i.e. $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$).\\

A function ${F}$ is s said to be safe if it is well-formed and full-invariant-by-Opponent.\\



\begin{defini}{(${F}$-Increasing Protocol)}\label{ProAbsCroi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification and $p$ be a protocol.\\
$p$ is ${F}$-increasing iff: $\forall R.r \in R_G(p), \sigma \in \Gamma,  \alpha \in {\mathcal{A}}(r^+), \mbox{ we have: }{F}(\alpha, r^+\sigma)\sqsupseteq \ulcorner \alpha \urcorner \sqcap{F}(\alpha, R^-\sigma)$
}
\end{defini}
$ $\\
An ${F}$-increasing protocol must produce traces with atomic messages having always a security level, returned by ${F}$, higher when sending (i.e. in $ r^+\sigma$) than when receiving (i.e. in $R^-\sigma$) or than its level set in the context (i.e. $\ulcorner \alpha \urcorner$), if known. \\


\begin{thm}{(Sececy in Increasing Protocols)}\label{mainTh}
{
Let ${F}$ be a safe function and $p$ be an ${F}$-increasing protocol.
\begin{center}
$p$ keeps its secret inputs.
\end{center}
}
\end{thm}
$ $\\

Theorem \ref{mainTh} states that a protocol keeps its secret inputs when it is analyzed by a safe function $F$ and is shown increasing. This result is quite intuitive. In fact, if the opponent succeeds to obtain a secret $\alpha$ (clear) from the protocol then its security level given  by $F$ is the infimum since $F$ is well-formed. That cannot be due to the rules of the protocol  since this latter is $F\mbox{-increasing}$. That could not arise neither when the opponent uses his capabilities since $F$ is full-invariant-by-opponent. So, the secret is kept forever. The detailed proof is available in~\cite{Relaxed}.

\section{Guideline for Building Safe Functions}\label{sectionFonctionsetSelections}


In ~\cite{WitnessArt1} we propose a class  of safe selections: $S_{Gen}^{EK}$. Any selection $S$ in $S_{Gen}^{EK}$ must return to an atom $\alpha$ in a message $m$:

\begin{enumerate}
\item if $\alpha$ is encrypted by a key $k$ such that $k$ is the outer key that satisfies the condition $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ (we refer to it by the external protective key), a subset among $k^{-1}$ and the neighbors of $\alpha$ under the same protection by $k$;
\item for two messages linked by a function $f$ in $\Sigma$ other than an encryption by a protective key (e.g. pair), the union of two subselections in these two messages.
\item if $\alpha$ does not have a protective key in $m$, the infimum (all atoms);
\item if $\alpha$ does not appear in $m$, the supremum (the empty set);
\end{enumerate}

%%We prove that any $S\in S_{Gen}^{EK}$ is ${\mathcal{C}}$-safe.\\

Among the selections of $S_{Gen}^{EK}$, we spotlight three practical ones:
\begin{enumerate}
\item the selection $S_{MAX}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$, all the principal identities inside the same protection by $k$, in addition to $k^{-1}$;
\item the selection $S_{EK}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$,  the key $k^{-1}$;
\item the selection $S_{N}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the key external protective key $k$, all the principal identities inside the same protection by $k$;
\end{enumerate}
Any selection $S$ in $S_{Gen}^{EK}$ when composed to a adequate homomorphism $\psi$ returns a safe function $F=\psi \circ S$. 
We choose the homomorphism that returns for:
\begin{enumerate}
\item an agent, its identity;
\item the key $k^{-1}$, if selected, the set of agent identities  that are authorized to know it.
\end{enumerate}
We denote by $F_{MAX}^{EK}, F_{EK}^{EK}$ and $F_{N}^{EK}$ respectively the functions resulting from the compositions $\psi \circ S_{MAX}^{EK}, \psi \circ S_{EK}^{EK}$ and $\psi \circ S_{N}^{EK}$. We prove~\cite{WitnessArt1} that these functions are safe. In fact, since the selection for any atom $\alpha$  is performed in an invariant section protected by the external protective key $k$, then, to alter this section (to decrease the security level of  $\alpha$), the opponent must have priorly obtained the atomic key $k^{-1}$. At this point of the proof, his knowledge must satisfy: $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner$. Since the key $ k^{-1}$ satisfies: $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ then the knowledge of the opponent must satisfy $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ too seeing that the comparator "$\sqsupseteq$" is transitive. This is simply the definition of a full-invariant-by-opponent function. These functions are well-formed by construction, too. 
%%\end{comment}


\begin{exemple}$ $\\

Context: $\ulcorner \alpha \urcorner=\{A, B, S\}$; $m=\{C.\{\alpha.D\}_{k_{as}}\}_{k_{ab}}$; ${k_{ab}^{-1}}={k_{ab}}, {k_{as}^{-1}}={k_{as}}$; $\ulcorner{k_{as}}\urcorner=\{A, S\}, \ulcorner{k_{ab}}\urcorner=\{A, B\}$. We have: \\
$S_{MAX}^{EK}(\alpha,m)=\{C, D, {k_{ab}^{-1}}\}$ and $F_{MAX}^{EK}(\alpha,m)=\psi\circ S_{MAX}^{EK}(\alpha,m)=\{C, D\}{ \cup}\ulcorner{k_{ab}^{-1}}\urcorner=\{C,D\} \cup \{A,B\}=\{A, B, C, D\}$.
\end{exemple} $ $\\

%%In all that follows, we refer to  any of the functions above by $F$ .

\section{Witness functions to eliminate the effect of variables}\label{sectionWF}

The functions  $F\in\{F_{MAX}^{EK}, F_{EK}^{EK}, F_{N}^{EK}\}$ we have  defined so far are not useful in practice since they operate on ground terms only. However, a static analysis should be run over messages of the generalized roles resulting from writing the protocol in a role-based specification~\cite{Debbabi11}. These messages contain variables that denote a content that an agent ignores and on which he cannot perform any verification. We give here a safe way to deal with variables. But now, let us  introduce derivation in Definition \ref{derivation}.$ $\\ %% as shown in \ref{derivation}. 
%%\pagebreak

\begin{defini}{[Derivation]}\label{derivation}
%%A derivative message is defined by the following rules:
%%\begin{table}[h]
%% \centering
\begin{center}
\begin{tabular}{rrcll}
~~~~~~& $\partial_X \alpha$ & $=$ & $\alpha$ &\\
& $\partial_X X$ & $=$& $\epsilon$ &\\
& $\!\!\partial_X Y~$ & $=$ & $Y, X\not = Y$ &\\
& $\partial{[\overline{X}]} m$ & $=$ & $\partial_{\{{\mathcal{X}}_m\backslash \{X\}\}} m$ &\\
& $\partial_X f(m)$ & $=$ & $ {f}(\partial_X m), f\in \Sigma$ &\\
& $\partial_{S_1 \cup S_2}m$ & $=$& $\partial_{S_1}\partial_{S_2}m$&\\ \\
\end{tabular}
\end{center}
%%\end{table}
\end{defini}

Derivation simply eliminates variables from a message except a variable under evaluation. The expression $\partial m$ denotes a message $m$ after removing all variables in. The aim of derivation is to deprive  variables from playing any role when evaluating an atom in a message. The idea  is hence to apply $F$ on the derivative message instead of the message itself. Besides, any variable is evaluated as a block with no regard to its content (i.e quantified). In fact, the reason why we do not care about the content of a variable is that if a variable, globally evaluated, is shown increasing that means that it cannot be discovered by any unauthorized party, and consequently any content inside cannot be discovered by an unauthorized party, too. If it is not increasing, then the protocol will not satisfy our sufficient conditions and hence no decision with respect to secrecy is made on, thus, with respect to authentication, too. This way of treating variables allows us to  give any content of a variable (dynamically known) the same value of the variable itself (statically calculable). The way we evaluate an atom from within a derivative message is described by Definition \ref{Fder}. $ $ \\
\begin{defini}\label{Fder}
$ $\\
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.\\
For all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, we denote by:
\[
F(\alpha, \partial [\overline{\alpha}] m\sigma) = \left\{
\begin{array}{ll}
F(\alpha,\partial m) & \mbox{if } \alpha \in {\mathcal{A}}(\partial m),\\
F(X,\partial [\overline{X}] m) & \mbox{if }\alpha \notin {\mathcal{A}}(\partial m) \\
%% & \mbox{and } \alpha \in {\mathcal{A}}(X\sigma). \\
& \mbox{and } \alpha =X\sigma. 
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma).\\
%% \underset{X \in {{\mathcal{X}}_m} } {\sqcap}

%% \mbox{ if } \alpha \not \in {\mathcal{A}}(\partial m) \mbox{ and }\alpha \in {\mathcal{A}}(X\sigma). \\
%% \\
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma). \\

\end{array}
\right.
\]
\end{defini}

Since the expression $F(\alpha, \partial [\overline{\alpha}] m\sigma)$ does not depend on substitution (i.e the run $\sigma$), we denote it simply by $F'(\alpha,m)$. Although the derivative function $F'$ allows us to neutralize variables, which is as such an important intermediate result, using it as is to analyze protocols is not safe because it is not even a function in the protocol. In fact, when we want to evaluate the security level of $\alpha$ in the trace $\{\alpha.A.B\}_{k_{cd}}­$ for example, we must return to the generalized roles to see from which message (with variables) this trace is generated and we may realize that more than one message are able to generate it. For instance, the messages $m_1=\{\alpha.A.X\}_{k_{cd}}­$ and $m_2=\{\alpha.Y.B\}_{k_{cd}}­$ are both candidates to generate the trace $\{\alpha.A.B\}_{k_{cd}}­$ (i.e. possible sources of it). If we refer to the first source (i.e. to $m_1$), the security level of $\alpha$ returned by $F'$ (with $F=F_{MAX}^{EK}$) is: 
$$F'(\alpha,\{\alpha.A.X\}_{k_{cd}})=F(\alpha,\{\alpha.\textcolor{red}{A}\}_{k_{\textcolor{red}{cd}}})=\{A, C, D\}$$
Whereas, if we refer to the second source (i.e. to $m_2$), its security level  is: 
$$F'(\alpha,\{\alpha.Y.B\}_{k_{cd}})=F(\alpha,\{\alpha.\textcolor{magenta}{B}\}_{k_{\textcolor{magenta}{cd}}})=\{B, C, D\}$$
Therefore, we cannot rely on $F'$ to analyze a protocol. To overcome this insufficiency, we define the witness functions. A witness function  looks for  all the sources of a ground term $m\sigma$ in the finite set  ${\mathcal{M}}_p^{\mathcal{G}}$, applies $F'$ to all of them, and returns the minimum. This minimum must satisfy both existence and uniqueness in the security lattice. Since a secret is always evaluated under the protection of a protective key, the research  of the  sources of a closed message in ${\mathcal{M}}_p^{\mathcal{G}}$ is then restricted to encryption patterns. We denote by  $\tilde{\mathcal{M}}_p^{\mathcal{G}}$ the set of all  encryption patterns generated by the protocol (renamed).\\


\begin{comment}
Let us see the problem in Example \ref{exempleApp}.

\begin{exemple}\label{exempleApp}
Let $m_1$ and $m_2$ be two messages of a generalized role such that 
$m_1=\{\alpha.C.X\}_{k_{ab}}$ and $m_2=\{\alpha.Y.S\}_{k_{ab}}$ and $\ulcorner\alpha\urcorner=\{A,B,S\}$ and $\ulcorner{k_{ab}^{-1}}\urcorner=\{A,B\}$. Let $m=\{\alpha.C.S\}_{k_{ab}}$ be a valid trace. Let $F=F_{MAX}^{EK}$.\\
$$F'(\alpha, m)=\begin{cases}
F'(\alpha, m_1\sigma_1)=\{A, B, C\}&| X\sigma_1=S\\
F'(\alpha, m_2\sigma_2)=\{A, B, S\}&| Y\sigma_2=C
\end{cases}$$
\end{exemple}

Thus, $F'$ is not compulsorily a function since it might return more than one output for the same input. 
\end{comment}




\begin{defini}{[witness function]}\label{WF}
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.
Let $p$ be a protocol and $F$ be a safe function. 
We define a witness function ${\mathcal{W}}_{p,F}$ for all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, as follows: 
%%On définit la fonction témoin sur les messages clos comme suit: 
\[{{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)=\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha, m'\sigma')\]
%%${\mathcal{W}}_{p,F}$ is said to be a witness function inside a protective key when $F$ is a verification Function such that its associated selection is an instance of the class $\Upsilon_{Gen}.$\\
\end{defini}

%%As we could see, a witness function depends on the set of sources of $m\sigma$ in ${\mathcal{M}}_p^{\mathcal{G}}$ (i.e. the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma|m'\sigma' = m \sigma\}$). So it depends on the substitution $\sigma$ that is not statically known. For that, we bind the witness function into two bounds that are independent of all substitution (runs). These bounds are provided by Lemma \ref{prePAT}.

Using a witness function as is to analyze a protocol is a very tedious  process since we cannot enumerate all the valid traces $m\sigma$ and their sources statically. For that we bind it into two bounds that do not depend on substitution (i.e on $\sigma$). The upper bound of a witness function returns a minimum set of confirmed principal identities for any $\alpha$ in $m$ whereas the lower bound returns the set of all principal identities from all the possible sources of $m$ (that are unifiable with it) including the odd ones.  The lower bound hunts so any odd principal identity and interprets it as an attack. The proof is simple since we have always  $\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma \} \subseteq \{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma' \}$ in the security lattice whatever $\sigma$. This is expressed by Proposition~\ref{prePAT}.\\

\begin{pre}{[binding a witness function]}\label{prePAT}
Let $m\in{\mathcal{M}}_p^{\mathcal{G}}$. Let ${\mathcal{W}}_{p,F}$ be a witness function.
For all $\sigma \in \Gamma$ we have:
$$F'(\alpha, m)\sqsupseteq {{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)\sqsupseteq \!\!\!\! \!\!\!\! \!\!\! \underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = m \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha, m'\sigma')$$
\end{pre}



\section{Sufficient conditions for authentication (Contribution)} \label{suffCondAuth}

The Lemma \ref{PAT} declares a decision criterion for secrecy  based on the bounds  of a witness function. The upper bound returns the set of original and trusted identities only from the received message. The lower bound returns the set of all the identities including those that could be inserted by a masquerader by substituting a regular message when sent. The criterion makes sure that no odd identity could be inserted in the evaluation neighborhood of a given  atom in the sent message.  The  proof  of Lemma \ref{PAT} results directly from Proposition \ref{prePAT} and Theorem \ref{mainTh}. \\

\begin{lem}{[Decision for Secrecy]}\label{PAT}
Let $p$ be a protocol. Let ${\mathcal{W}}_{p,F}$ be a witness function.
$p$ is correct with respect to secrecy if:
$\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$ we have:
$$\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}}\otimes\Gamma|m'\sigma' = r^+ \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F'(\alpha,  m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F'(\alpha, R^-)$$
\end{lem}

Theorem \ref{PAT2} forwards two conditions such, if met, a protocol is automatically declared correct for authentication. The first one ensures that the protocol does not disclose its secret inputs. An immediate outcome of this first result is that the message the verifier last receives for authentication is in a safe state and had not been subverted by a masquerader. The second one makes sure that the binding between the challenge and the identity of the identifier is not cut.  Therefore, we call once again the upper bound of the witness function to confirm the originality of the claimer identity by evaluating the challenge in the  message that should authenticate the claimer to the verifier. The second clause of the second condition is trivial  and introduced just to make sure that the challenge is not received in a public state.\\

\begin{thm}{[Decision for Authentication]}\label{PAT2}
Let $p$ be a protocol. Let ${\mathcal{W}}_{p,F}$ be a witness function.
$p$ is correct with respect to authentication if:
\begin{enumerate}
\item Lemma \ref{PAT} is satisfied;
\item Let $\alpha$ be the challenge in a message $m$ received by a verifier $B$ to authenticate an agent $A$. We  have:
$$A \in F'(\alpha, m)  \wedge F'(\alpha,  m)  \sqsupset \bot$$
\end{enumerate}
\end{thm}
It is worth mentioning  that:
\begin{itemize}
 
\item  the conditions set by Theorem \ref{PAT2} can be verified statically as they use the two bounds of a witness function only and  both of them are statically determinable;
\item their verification is linear under the assumption of perfect encryption since the most costly operation is unification in the lower bound of a witness function which is linear under that assumption. However, under nonempty equational theories, it will vary from one to another. In a future work, we will give new results related to this question.
   
\end{itemize}

==> someProtocol.tex <==





\section{Protocol Definition and Context Setup}  \label{sectionAnWL2}

We analyze the protocol defined by $p$ in Table~\ref{WLMV:protv2p} for secrecy. The aim of our analysis is to prove that $p$ does not divulge the secret $sec$, supposed to be exposed to $A$ and $S$ only. We show that the interpretation-Functions fail, where a Witness-Function succeeds.

\begin{center}
          \begin{table}[h]
      \begin{center}    
         \caption{Protocol Definition}
         \label{WLMV:protv2p} 
               $\begin{array}{|l|}
               \hline\\
                   \begin{array}{llll}
                    p   :=&\langle 1,A\rightarrow S: \{A.N_a.S.B\}_{k_s}\rangle.  \\
                    & \langle 2,S\rightarrow B: \{B.A.S.N_a\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}\rangle. \\
                    & \langle 3,B\rightarrow A:\{B.\{S.sec\}_{k_a}.A.N_a.S\}_{k_{a}}\rangle\\ &\\
                    \end{array} \\ \hline  \end{array}$
\end{center}
         \end{table}
\end{center}

    The   role-based   specification  of $p$  is ${\cal R}_G(p) = \{{\cal A}_G ,~{\cal B}_G ,~ {\cal S}_G \}$,
    where the generalized role ${\cal A}_G $ of $A$ is as follows:
    \[\begin{array}{l}
             \begin{array}{llllll}
                    {\cal A}_G =& \langle  i.1,  A    & \rightarrow & I(S):&  \{A.N_a^{i}.S.B\}_{k_s} \rangle.\\
                    & \langle i.2,  I(B)    & \rightarrow & A:&  \{B.\{S.X\}_{k_a}.A.N_a^{i}.S\}_{k_{a}}\rangle
             \end{array}\end{array}\]

     The generalized role ${\cal B}_G $  of $B$ is as follows:
            \[\begin{array}{l}
            \begin{array}{lllll}
                {\cal B}_G =& \langle i.1,  I(S) & \rightarrow & B:& \{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b} \rangle.\\
                        & \langle i.2,  B    & \rightarrow & I(A) :&  \{B.Z.A.Y.S\}_{k_{a}} \rangle  \\
            \end{array}
             \end{array}\]

             The  generalized role $ {\cal S}_G$ of $S$ is as follows:
            \[\begin{array}{l}
             \begin{array}{lllll}
                            {\cal S}_G = & \langle i.1, I(A) & \rightarrow & S:& \{A.T.S.B\}_{k_s}
                             \rangle. \\
                                    & \langle i.2,S & \rightarrow & I(B):&\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}\rangle\\
               \end{array}
            \end{array} \]
            
Let us have a context of verification such that: \\

$\ulcorner k_{a}\urcorner=\ulcorner k_{b}\urcorner = \ulcorner k_{s}\urcorner=\bot$ (public keys); 

$\ulcorner k_{a}^{-1}\urcorner = \{A\}$; $\ulcorner k_{b}^{-1}\urcorner = \{B\}$; $\ulcorner k_{s}^{-1}\urcorner = \{S\}$ (private keys);

$\ulcorner N_a^i \urcorner=\{A, B, S\}$ (nonce shared between $A, B$ and $S$); 

$\ulcorner sec \urcorner=\{A, S\}$ (secret shared between $A$ ans $S$ \textbf{\underline{only}}); 

$\forall \mbox{ agID } \in {\cal{I}}, \ulcorner \mbox{ agID } \urcorner=\bot$ (agents' identities are public);

The variables are denoted by $X$, $Y$, $Z$ and $T$ in the generalized roles.\\

%%The principal identities are not analyzed since they are set public in the context.\\

 
%After eliminating   duplicates in ${\cal{M}}_{p}^{\cal{G}}$ and the messages that are not encryption patterns, we have:\\ $ $\\
%$\tilde{\cal{M}}_{p}^{\cal{G}}= \{
%\{B_1.K_{A_{2}B_{1}}^i\}_{K_{A_{2}S_{1}}},
%\{A_4.N_{B_{3}}^i.Y_2 \}_{K_{{B_{3}S_2}}},$ $
%\{N_{B_{4}}^i.\{A_5.Z_1\}_{K_{B_{4}S_3}}\}_{K_{B_{4}S_3}},
%\{A_6.U_1.\{B_5.V_1\}_{K_{{A_6}S_4}}\}_{K_{{B_5}S_4}},\\
%\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}}
% \}$\\
 

\section{Protocol analysis with the Interpretation-Functions} \label{sectionAnWL222}

For the sake of conciseness, we do not analyze the entire protocol. We analyze just the generalized role of $B$ where the Interpretation-Functions fail to show the growth of the protocol. In that generalized role, $B$ receives $R^{-}=\{A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b}$ and sends $r^{+}=\{B.Z.A.Y\}_{k_{a}}$. 

\subsection{Analysis with the DEK function} \label{sectionAnWL5486}
\begin{enumerate}

\item Receiving step: $\mbox{DEK}(Y,R^{-}) = \mbox{DEK}(Y, \{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b})=$ $\mbox{DEK}(Y, \{B.A.S.Y\}_{k_b}) \sqcap \mbox{DEK}(Y, \{A.B.S.Z\}_{k_b})=$ $\ulcorner k_b^{-1} \urcorner \sqcap \top=\ulcorner k_b^{-1} \urcorner=\{B\}$
\item Sending step: $\mbox{DEK}(Y,r^{+}) = \mbox{DEK}(Y, \{B.Z.A.Y.S\}_{k_{a}})=\ulcorner k_a^{-1} \urcorner=\{A\}$
\end{enumerate}
As we can see, we cannot prove that $\mbox{DEK}(Y,r^{+})  \sqsupseteq \ulcorner Y \urcorner \sqcap \mbox{DEK}(Y,R^{-})$. So, the DEK function fails.

\subsection{Analysis with the \mbox{DEKAN} function} \label{sectionAnWL877}

\begin{enumerate}

\item On receiving: $\mbox{DEKAN}(Y,R^{-}) = \mbox{DEKAN}(Y, \{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b})=$ $\mbox{DEKAN}(Y, \{B.A.S.Y\}_{k_b}) \sqcap \mbox{DEKAN}(Y, \{A.B.S.Z\}_{k_b})=$ $\ulcorner k_b^{-1} \urcorner \sqcap \{ B, A, S\} \sqcap \top=\ulcorner k_b^{-1} \urcorner  \sqcap \{B, A, S\} =\{B\} \cup \{B, A, S\}=  \{A, B, S\}$
\item On sending: $\mbox{DEKAN}(Y,r^{+}) = \mbox{DEKAN}(Y, \{B.Z.A.Y.S\}_{k_{a}})=\ulcorner k_a^{-1} \urcorner \cup \{B, Z, A, S\}=\{B, Z, A, S\}$
\end{enumerate}
As we can see, we cannot prove that $\mbox{DEKAN}(Y,r^{+})  \sqsupseteq \ulcorner Y \urcorner \sqcap \mbox{DEKAN}(Y,R^{-})$. So, the DEKAN function fails, as well.


\section{Protocol analysis with the Witness-Functions} \label{sectionAnWL222333}

Let $F= F_{MAX}^{IK}$; ${\mathcal{W}}_{p,F}= {\mathcal{W}}_{{p},F_{MAX}^{IK}}$;\\

We denote  by ${\Upsilon}_{p,F}(\alpha,m)$ the lower bound $\underset{\{{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}}\otimes \Gamma{|m'\sigma' = m\sigma' \}}}{\sqcap}\!\!\!\!\!\!\!\!\!\!  F'(\alpha, m'\sigma')$ of the witness function ${\mathcal{W}}_{p,F}(\alpha,m)$.\\

The set of encryption patterns generated by $p$ is  $\tilde{\cal{M}}_{p}^{\cal{G}}=\{
 \{A_1.N_{A_1}.S_1.B_1\}_{K_{S_1}},
\{B_2.\{S_2.X_2\}_{K_{A_2}}.A_2.N_{A_2}.S_2\}_{K_{A_2}},\\
\{B_3.A_3.S_3.Y_3\}_{K_{B_3}}, \{A_4.B_4.S_4.Z_4\}_{K_{B_4}},\\
 \{B_5.Z_5.A_5.Y_5.S_5\}_{K_{A_5}},\\ \{A_6.T_6.S_6.B_6\}_{K_{S_6}}, 
 \{B_7, A_7.S_7.T_7\}_{K_{B_7}},\\ \{A_8.B_8.S_8.\{S_8.sec_8\}_{K_{A_8}}\}_{K_{B_8}}
 \}$\\
 
 The renamed variables in $\tilde{\cal{M}}_{p}^{\cal{G}}$ are denoted by $X_2, Y_3, Z_4, Z_5, Y_5, T_6$ and $T_7$;\\ 

\subsection{Analysis of the Generalized Roles of $A$}

According to the generalized role of  $A$, an agent $A$ may take part in some session $S^{i}$  in which he receives nothing (i.e. $\epsilon$) and sends the message $\{A.N_a^{i}.S.B\}_{k_s}$. This is described by the following rule: \[{S^{i}}:\frac{\epsilon}{ \{A.N_a^{i}.S.B\}_{k_s}}\]

\noindent{-Analysis of the messages exchanged  in $S^{i}$:}\\
\\
1- For $N_a^{i}$:\\

a- Receiving step: $R_{S^{i}}^-=\epsilon$ \textit{(when receiving, we use the upper bound)}

\begin{equation}
F'(N_a^{i}, R_{S^{i}}^-)=F(N_a^{i},\partial  [\overline{N_a^{i}}]\epsilon)=F(N_a^{i},\epsilon)=\top
\label{eq1}
\end{equation}

b- Sending step: $r_{S^{i}}^+= \{A.N_a^{i}.S.B\}_{k_s}$ \textit{(when sending , we use the lower bound)}\\

Since $\{A.N_a^{i}.S.B\}_{k_s}$ is a ground term (no variable in), then we have: ${\Upsilon}_{p,F}(N_a^{i}, \{A.N_a^{i}.S.B\}_{k_s})= $ $F(N_a^{i}, \{A.N_a^{i}.S.B\}_{k_s})$\\

$\mbox{Since } F=F_{MAX}^{IK}$, we have:\\

$F(N_a^{i}, \{A.N_a^{i}.S.B\}_{k_s})=\ulcorner k_{s}^{-1} \urcorner \cup \{A, S, B\}$. Then:\\

\begin{equation}
{\Upsilon}_{p,F}(N_a^{i}, \{A.N_a^{i}.S.B\}_{k_s})=\{A, S, B\} \label{eq2}
\end{equation}
\\
2- Conformity  with Theorem \ref{PAT}:\\ 

From (\ref{eq1}) and (\ref{eq2}) and since $ \ulcorner N_a^{i} \urcorner=\{A, B, S\}$ in the context, we have:
\begin{equation}
{\Upsilon}_{p,F}(N_a^{i}, r_{S^{i}}^+) \sqsupseteq \ulcorner N_a^{i} \urcorner \sqcap F'(N_a^{i}, R_{S^{i}}^-)
\label{eq3}
\end{equation}


%%(1.2)\\
Then,  the generalized role of $A$ respects Theorem \ref{PAT}. ~~~~ (I)


\subsection{Analysis of the generalized roles of $B$}
According to the generalized role of $B$, an agent $B$ participates in a session $S^{i}$ in which he receives the message $\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b}$ and sends the message $\{B.Z.A.Y.S\}_{k_{a}}$. This is described by the following rule:

\[{S^{i}}:\frac{\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b}}{\{B.Z.A.Y.S\}_{k_{a}}}\]
$ $\\

1-$\forall Z$:\\

a- Receiving step: $R_{S^{i}}^-=\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b}$ \textit{(when receiving, we use the upper bound)}

\begin{equation} 
\begin{tabular}{lll}
   $F'(Z,R_{S^{i}}^-)$  &$=$& $F'(Z,\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b} )$\\
    & $=$ & $F(Z,\partial  [\overline{Z}]\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b})$  \\
   & $=$ & $F(Z,\{B.A.S\}_{k_b}.\{A.B.S.Z\}_{k_b} )$ \\
   & $=$ & $ F(Z,\{B.A.S\}_{k_b}) \sqcap F(Z,\{A.B.S.Z\}_{k_b} )  $ \\
    & $=$  & $\top \sqcap  F(Z,\{A.B.S.Z\}_{k_b} ) $ \\
    & $=$  & $ F(Z,\{A.B.S.Z\}_{k_b} ) $ \\
    & $=$  & $\ulcorner k_{b}^{-1} \urcorner \cup \{A,B, S\} $ \\
    & $=$  & $\{A, B, S\}$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq4}
\end{equation}

%Since $N_b^i$ is set public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then, we have directly:
%\begin{equation}
%{\Upsilon}_{p,F}(N_b^i,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner N_b^i \urcorner \sqcap  F'(N_b^i,Y )\\
%\label{eq5}
%\end{equation}

b- Sending step: $r_{S^{i}}^+=\{B.Z.A.Y.S\}_{k_{a}}$ \textit{(when sending , we use the lower bound)}\\

 $\forall Z.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\
 
 $=\forall Z.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = \{B.Z.A.Y.S\}_{k_{a}} \sigma' } \}$ \\
 
 $=\{(  \{B_5.Z_5.A_5.Y_5.S_5\}_{K_{A_5}},\sigma_1')\}$ such that: 
 
 $\sigma_1'=\{ B_5 \longmapsto B, Z_5\longmapsto Z, A_5 \longmapsto A, Y_5 \longmapsto Y,$\\  $~~~~~~~~~~~~~S_5 \longmapsto S, K_{A_{5}}\longmapsto  k_{a}\}$\\
 

${\Upsilon}_{p,F}(Z,\{B.Z.A.Y.S\}_{k_{a}})$\\

$=\{\mbox{Definition of the lower bound of the witness function}\}$\\

$F'(Z,\{B_5.Z_5.A_5.Y_5.S_5\}_{K_{A_5}} \sigma_{1}') $\\

$=\{\mbox{Setting the static neighborhood}\}$\\

$F'(Z, \{B.Z_5.A.Y.S\}_{k_{a}} \sigma_{1}')$ \\

$=\{\mbox{Definition } \ref{Fder}\}$\\

$F(Z_5,\partial[\overline{Z_5}]  \{B.Z_5.A.Y.S\}_{k_{a}})$ \\

%%$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\
$=\{\mbox{Derivation in Definition } \ref{derivation}\}$
\\

$F(Z_5, \{B.Z_5.A.S\}_{k_{a}})$ \\

$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\

$\ulcorner k_{a}^{-1} \urcorner \cup \{B, A, S\}=\{A, B, S\}$\\%%(3.2)\\

Then, we have:

\begin{equation}
{\Upsilon}_{p,F}(Z,\{B.Z.A.Y.S\}_{k_{a}})=\{A, B, S\}
\label{eq5}
\end{equation}


2- $\forall Y$:\\

a- Receiving step: $R_{S^{i}}^-=\{A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b}$ \textit{(when receiving, we use the upper bound)}

\begin{equation} 
\begin{tabular}{lll}
   $F'(Y,R_{S^{i}}^-)$  &$=$& $F'(Y,\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b} )$\\
    & $=$ & $F(Y,\partial  [\overline{Y}]\{B.A.S.Y\}_{k_b}.\{A.B.S.Z\}_{k_b})$  \\
   & $=$ & $F(Y,\{B.A.S.Y\}_{k_b}.\{A.B.S\}_{k_b} )$ \\
   & $=$ & $ F(Y,\{B.A.S.Y\}_{k_b}) \sqcap F(Y,\{A.B.S\}_{k_b} )  $ \\
   & $=$ & $ F(Y,\{B.A.S.Y\}_{k_b}) \sqcap\top  $ \\
   & $=$ & $ F(Y,\{B.A.S.Y\}_{k_b})$ \\
    & $=$  & $\ulcorner k_{b}^{-1} \urcorner \cup \{B, A, S\} $ \\
    & $=$  & $\{A, B, S\}$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq6}
\end{equation}

%Since $N_b^i$ is set public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then, we have directly:
%\begin{equation}
%{\Upsilon}_{p,F}(N_b^i,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner N_b^i \urcorner \sqcap  F'(N_b^i,Y )\\
%\label{eq5}
%\end{equation}

b- Sending step: $r_{S^{i}}^+=\{B.Z.A.Y.S\}_{k_{a}}$ \textit{(when sending , we use the lower bound)}\\

 $\forall Y.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\
 
 $=\forall Y.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = \{B.Z.A.Y.S\}_{k_{a}} \sigma' } \}$ \\
 
 $=\{(  \{B_5.Z_5.A_5.Y_5.S_5\}_{K_{A_5}},\sigma_1')\}$ such that: 
 
 $\sigma_1'=\{ B_5 \longmapsto B, Z_5\longmapsto Z, A_5 \longmapsto A, Y_5 \longmapsto Y,$\\  $~~~~~~~~~~~~~S_5 \longmapsto S, K_{A_{5}}\longmapsto  k_{a}\}$\\
 

${\Upsilon}_{p,F}(Y, \{B.Z.A.Y.S\}_{k_{a}})$\\

$=\{\mbox{Definition of the lower bound of the witness function}\}$\\

$F'(Y, \{B_5.Z_5.A_5.Y_5.S_5\}_{K_{A_5}} \sigma_{1}') $\\

$=\{\mbox{Setting the static neighborhood}\}$\\

$F'(Y, \{B.Z.A.Y_5.S\}_{k_{a}} \sigma_{1}')$ \\

$=\{\mbox{Definition } \ref{Fder}\}$\\

$F(Y_5,\partial[\overline{Y_5}]  \{B.Z.A.Y_5.S\}_{k_{a}})$ \\

%%$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\
$=\{\mbox{Derivation in Definition } \ref{derivation}\}$
\\

$F(Y_5, \{B.A.Y_5.S\}_{k_{a}})$ \\

$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\

$\ulcorner k_{a}^{-1} \urcorner \cup \{B, A, S\}=\{A, B, S\}$\\%%(3.2)\\

Then, we have:

\begin{equation}
{\Upsilon}_{p,F}(Y,\{B.Z.A.Y.S\}_{k_{a}})=\{A, B\}
\label{eq7}
\end{equation}

3- Conformity  with Theorem \ref{PAT}:\\

From (\ref{eq4}) and (\ref{eq5}), we have:
\begin{equation}
{\Upsilon}_{p,F}(Z, r_{S^{i}}^+) \sqsupseteq \ulcorner Z \urcorner \sqcap F'(Z, R_{S^{i}}^-)
\label{eq8}
\end{equation}

From (\ref{eq6}) and (\ref{eq7}), we have:
\begin{equation}
{\Upsilon}_{p,F}(Y, r_{S^{i}}^+) \sqsupseteq \ulcorner Y \urcorner \sqcap F'(Y, R_{S^{i}}^-)
\label{eq9}
\end{equation}

From (\ref{eq8}) and (\ref{eq9}), we have:  the generalized role of $B$ respects Theorem \ref{PAT}. ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(II)\\

\subsection{Analysis of the generalized roles of $S$}$ $\\

According to the generalized role of $B$, an agent $B$ participates in a session $S^{i}$ in which he receives the message $\{A.T.S.B\}_{k_s}$ and sends the message $\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}$. This is described by the following rule:

\[{S^{i}}:\frac{\{A.T.S.B\}_{k_s}}   {\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}}\]
$ $\\

1- $\forall T$:\\

a- Receiving step: $R_{S^{i}}^-=\{A.T.S.B\}_{k_s}$ \textit{(when receiving, we use the upper bound)}

\begin{equation} 
\begin{tabular}{lll}
   $F'(T,\{A.T.S.B\}_{k_s})$ & $=$ & $F(T,\partial  [\overline{T}]\{A.T.S.B\}_{k_s})$  \\
   & $=$ & $ F(T,\{A.T.S.B\}_{k_s} )$ \\
    & $=$  & $\ulcorner k_{s}^{-1} \urcorner \cup \{A, S, B\} $ \\
    & $=$  & $\{A, B, S\}$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq10}
\end{equation}

b- Sending step: $r_{S^{i}}^+=\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}$ \textit{(when sending , we use the lower bound)}\\
We have: 

\begin{equation}
\begin{tabular}{lll}
   ${\Upsilon}_{p,F}(T,r_{S^{i}}^+)$ & $=$ & ${\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$  \\
   & $=$ & ${\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b}) \sqcap$ \\
   & $ $ & ${\Upsilon}_{p,F}(T,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}) $ \\
   & $=$ & ${\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b}) \sqcap \top$ \\
   & $=$ & ${\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b})$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq11}
\end{equation}

 $\forall T.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\
 
 $=\forall T.\{(m',\sigma') \in \tilde{\cal{M}}_{p}^{\cal{G}}\otimes\Gamma|{m'\sigma' = \{B.A.S.T\}_{k_b}\}_{k_{bs}} \sigma' } \}$ \\
 
 $=\{(\{A_7.S_3.Y_1\}_{K_{B_2}},\sigma_1')\}$ such that: 
 
 $$\sigma_1'=\{ B_7 \longmapsto B, A_7 \longmapsto A, S_7 \longmapsto S, T_7 \longmapsto T, K_{B_{7}}\longmapsto  k_{b}\}$$\\
 

${\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b})$\\

$=\{\mbox{Definition of the lower bound of the witness function}\}$\\

$F'(T,\{B_7.A_7.S_7.T_7\}_{K_{B_4}}\sigma_{1}') $\\

$=\{\mbox{Setting the static neighborhood}\}$\\

$F'(T, \{B.A.S.T_7\}_{k_{b}} \sigma_{1}')$ \\

$=\{\mbox{Definition } \ref{Fder}\}$
\\

$F(T_7,\partial[\overline{T_7}] \{B.A.S.T_7\}_{k_{b}})$ \\

%%$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\
$=\{\mbox{Derivation in Definition } \ref{derivation}\}$
\\

$F(T_7,\{B.A.S.T_7\}_{k_{b}})$ \\

$=\{\mbox{Since } F=F_{MAX}^{IK}\}$\\

$\ulcorner k_{b}^{-1} \urcorner \cup \{B, A, S\}=\{A, B, S\}$\\%%(3.2)\\

Then, we have:

\begin{equation}
{\Upsilon}_{p,F}(T,\{B.A.S.T\}_{k_b})=\{A, B, S\}
\label{eq12}
\end{equation}

2- For the secret $sec$:\\

a- Receiving step: $R_{S^{i}}^-=\{A.T.S.B\}_{k_s}$ \textit{(when receiving, we use the upper bound)}\\

\begin{equation} 
\begin{tabular}{lll}
   $F'(sec,\{A.T.S.B\}_{k_s})$ & $=$ & $F(sec,\{A.S.B\}_{k_s})$  \\
   & $=$ & $\top$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq13}
\end{equation}

b- Sending step: $r_{S^{i}}^+=\{B.A.S.T\}_{k_b}.\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}$ \textit{(when sending , we use the lower bound)}\\

\begin{equation}
\begin{tabular}{lll}
   ${\Upsilon}_{p,F}(sec,r_{S^{i}}^+)$ & $=$ & ${\Upsilon}_{p,F}(sec,\{B.A.S.T\}_{k_b}.$  \\
    & & $\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$  \\
   & $=$ & ${\Upsilon}_{p,F}(sec,\{B.A.S.T\}_{k_b}) \sqcap$ \\
   & $ $ & ${\Upsilon}_{p,F}(sec,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b}) $ \\
   & $=$ & $\top \sqcap {\Upsilon}_{p,F}(sec,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$ \\
   & $=$ & ${\Upsilon}_{p,F}(sec,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$ \\
\end{tabular}
%%F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )= F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\} %%$ (3.2)\\
\label{eq14}
\end{equation}

Since $\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$ is a ground term, we have directly:

\begin{equation}
\begin{tabular}{lll}
   ${\Upsilon}_{p,F}(sec,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$ & $=$ &   \\
   $F(sec,\{A.B.S.\{S.sec\}_{k_a}\}_{k_b})$ & $=$ & \\ 
     $~~~~~~~~~~~~~~~~~~~~~~\{\mbox{Since } F=F_{MAX}^{IK}\}$ & &\\ 
  $\ulcorner {k_a}^{-1}\urcorner \cup \{S\} $ & $=$ & $\{A, S\}$ 
\end{tabular} 
\label{eq15}
\end{equation}

3- Conformity  with Theorem \ref{PAT}:\\


From (\ref{eq10}) and (\ref{eq12}), we have:\\
\begin{equation}
{\Upsilon}_{p,F}(T,r_{S^{i}}^+) \sqsupseteq \ulcorner T \urcorner \sqcap F'(T,R_{S^{i}}^- )
\label{eq16}
\end{equation}

From (\ref{eq13}) and (\ref{eq15}), we have:\\
\begin{equation}
{\Upsilon}_{p,F}(sec,r_{S^{i}}^+) \sqsupseteq \ulcorner sec \urcorner \sqcap F'(sec,R_{S^{i}}^- )
\label{eq17}
\end{equation}

From (\ref{eq16})  and (\ref{eq17}),  we have:  the generalized role of $S$ respects Theorem \ref{PAT}. ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(III)$ $\\


From (I) and (II) and (III), we conclude that: $p$ respects Theorem~\ref{PAT}. So it is increasing, then, it is correct for secrecy. ~~~~(IV)\\

